Leveraging Generative AI for Urban Digital Twins: A Scoping Review on the Autonomous Generation of Urban Data, Scenarios, Designs, and 3D City Models for Smart City Advancement

The digital transformation of modern cities by integrating advanced information, communication, and computing technologies has marked the epoch of data-driven smart city applications for efficient and sustainable urban management. Despite their effectiveness, these applications often rely on massive amounts of high-dimensional and multi-domain data for monitoring and characterizing different urban sub-systems, presenting challenges in application areas that are limited by data quality and availability, as well as costly efforts for generating urban scenarios and design alternatives. As an emerging research area in deep learning, Generative Artificial Intelligence (AI) models have demonstrated their unique values in data and code generation. This survey paper aims to explore the innovative integration of generative AI techniques and urban digital twins to address challenges in the realm of smart cities in various urban sectors, such as transportation and mobility management, energy system operations, building and infrastructure management, and urban design. The survey starts with the introduction of popular generative AI models with their application areas, followed by a structured review of the existing urban science applications that leverage the autonomous capability of the generative AI techniques to facilitate (a) data augmentation for promoting urban monitoring and predictive analytics, (b) synthetic data and scenario generation, (c) automated 3D city modeling, and (d) generative urban design and optimization. Based on the review, this survey discusses potential opportunities and technical strategies that integrate generative AI models into the next-generation urban digital twins for more reliable, scalable, and automated management of smart cities.

==> Content/000-aiding-materials.tex <==

Conditional CycleGANs represent an innovative advancement in the realm of image-to-image translation, an area where Generative Adversarial Networks (GANs) have already made significant strides. Building upon the principles of CycleGANs , which facilitated the transformation of images from one domain to another without paired examples, Conditional CycleGANs incorporate conditional information, such as class labels or attributes, to guide the image translation process. This addition enables more precise control over the characteristics of the transformed images, allowing for tailored and context-specific outputs. The genesis of Conditional CycleGANs is rooted in the need for more nuanced and controlled image translation in diverse applications. These networks have found extensive use in various domains. In artistic endeavors, they assist in style transfer and photo-realistic rendering, enabling artists to transform images in line with specific styles or themes. In medical imaging, they aid in generating more accurate synthetic images for training and diagnostic purposes, respecting critical details influenced by conditional parameters. In the realm of augmented reality and virtual reality, Conditional CycleGANs contribute to creating more immersive and realistic environments by adapting visual elements to user-specified conditions. The flexibility and precision of Conditional CycleGANs in handling complex image translation tasks make them a potent tool in advancing both academic research and practical applications across multiple fields.



They can be employed in urban planning to create detailed simulations and visualizations of urban environments, aiding in decision-making and public engagement processes. 

In traffic management, these models can help simulate a range of traffic scenarios, assisting in the optimization of traffic flow and public transportation routes. 

Additionally, in environmental monitoring, Diffusion Models can be used to predict changes in urban environmental conditions, such as air quality and noise levels, based on various urban development scenarios. 

Furthermore, they can contribute to energy management by modeling and forecasting energy consumption patterns in urban areas, leading to more efficient energy usage. T

The article "Diffusion Models: A Comprehensive Survey of Methods and Applications" presents a detailed overview of diffusion models, focusing on their development, methodologies, and diverse applications. The authors categorize research on diffusion models into three primary areas: efficient sampling, improved likelihood estimation, and handling data with special structures. They explore various techniques and advancements within these categories, highlighting the significance of diffusion models in fields like computer vision, natural language processing, and interdisciplinary scientific applications. The review also discusses the potential integration of diffusion models with other generative models for enhanced performance, providing an insightful perspective for both new and experienced researchers in this evolving field.


%For example, in urban planning, VAEs can be utilized to generate diverse urban layouts and architectural models, aiding in the exploration of various design alternatives. In traffic management, they can assist in predicting traffic patterns and simulating the impact of urban interventions, thereby informing better traffic and transportation policies. Additionally, VAEs have potential applications in energy management, where they can be employed to model and predict energy consumption patterns across different urban sectors, leading to more efficient energy distribution and conservation strategies. Furthermore, their application in environmental monitoring allows for the prediction and simulation of environmental conditions, aiding in proactive urban management decisions. 


\subsection{Autoregressive Models} 
\label{subsec:autoregressive-models}
Autoregressive Models, fundamental tools in statistical analysis and signal processing, have been instrumental in modeling and predicting time-dependent data. The concept, which dates back to the early 20th century with roots in the work of Yule (1927) on time series analysis, revolves around using previous values in a time series to predict future values. This predictive capability stems from the model's inherent design, where the current value of a series is regressed on its own prior values. In the evolution of smart city technologies, Autoregressive Models have found a wide array of applications. Their ability to analyze and forecast time-series data makes them particularly suitable for urban traffic management, where they can predict traffic flow and congestion patterns, aiding in efficient traffic control and planning. In energy management, these models are utilized to forecast demand and supply, contributing to more effective and sustainable energy utilization. Autoregressive Models also play a critical role in environmental monitoring, predicting pollution levels and environmental changes over time, thereby assisting in proactive urban environmental management. Furthermore, in the realm of public safety, they aid in predicting crime trends, enabling smarter and more responsive urban policing strategies. The versatility and precision of Autoregressive Models in handling temporal data make them a key component in the data-driven management and optimization of modern smart cities.



handling large volumes of data.

This interest is evident in the expanding use of transformers for data discovery, where they enable more nuanced and accurate analysis of textual data across diverse domains. Moreover, the application of transformer-based models in creating autonomous research tools is a significant leap forward. These tools, equipped with the capability to understand and generate code, are aiding researchers and data scientists in automating tedious coding tasks, thus accelerating the pace of research and analysis. The transformative impact of these models in various scientific fields underscores their potential as a pivotal technology in the ongoing quest for more advanced and efficient data processing and analysis methodologies.

Transformer-Based Models, a paradigm-shifting development in the field of machine learning, have revolutionized the way we approach complex data processing tasks. Introduced by Vaswani et al. in their 2017 landmark paper, 'Attention is All You Need', these models marked a departure from the traditional recurrent neural network architectures, offering a more efficient and scalable approach to handling sequential data. Central to transformers is the mechanism of self-attention, which allows the model to weigh the significance of different parts of the input data independently, leading to a more nuanced and context-aware processing. This architectural innovation has had profound implications in various applications, particularly in natural language processing. In the context of smart city applications, Transformer-Based Models offer significant potential. They can be employed in analyzing and interpreting large volumes of urban data, such as traffic patterns, social media feeds, and sensor data, facilitating more informed decision-making in urban planning and management. In traffic and transportation management, transformers can help in optimizing routes and predicting congestion, thereby enhancing traffic flow and public transportation systems. In environmental monitoring, these models can process complex environmental data to predict pollution levels and assess the impact of urban activities on air quality. Additionally, their application in public safety can involve analyzing patterns in crime data and emergency response records, aiding in the development of more effective public safety strategies. The power and versatility of Transformer-Based Models lie in their ability to process vast and varied data streams, making them an invaluable asset in the development of responsive, efficient, and intelligent smart city systems.

%ChatGPT is based on the GPT (Generative Pre-trained Transformer) architecture, which is indeed a transformer-based model. The transformer architecture is fundamental in ChatGPT, enabling it to understand and generate human-like text by processing words in relation to all other words in a sentence, rather than one-by-one in order. This allows for more fluid and context-aware responses in conversations.


In the rapidly evolving domain of urban development, 3D city modeling has emerged as a pivotal technology, reshaping our approach to conceptualizing and realizing the vision of smart cities. At its core, 3D city modeling involves the creation of digital representations of urban areas, capturing the physical dimensions and geographical elements in three-dimensional space. This technology serves as a critical tool for urban planners, architects, and policymakers, providing a detailed and scalable view of city landscapes. The value of 3D city modeling lies in its ability to facilitate informed decision-making and efficient resource management, essential for the sustainable development of smart cities. By enabling simulations and analyses of various urban scenarios, this technology aids in optimizing land use, improving infrastructure planning, and enhancing public safety. Furthermore, 3D city models are instrumental in engaging stakeholders and the public, offering interactive visualizations that aid in understanding complex urban dynamics. The applications of 3D city modeling extend to various sectors, including transportation management, where it assists in traffic flow analysis and public transit planning, and environmental monitoring, where it aids in assessing the impact of urbanization on local ecosystems. Additionally, in the realm of disaster management, 3D city modeling proves invaluable in risk assessment and emergency response planning. The integration of 3D city models with emerging technologies such as the Internet of Things (IoT), artificial intelligence (AI), and big data analytics further amplifies their potential, paving the way for more adaptive, efficient, and responsive urban environments. Thus, 3D city modeling is not only a facilitator of urban innovation but also a cornerstone in the quest to build smarter, more sustainable cities.



These applications demonstrate how cognitive digital twins are not just replicating physical entities but are also evolving with intelligent, data-driven insights, significantly contributing to the development of smarter, more responsive urban environments.


\subsection{Digital Twins Technological Framework} 
Key components of digital twins include:
\begin{enumerate}
    \item Data Collection Layer: Sensors and IoT devices that collect real-time data from the physical asset.
    \item Communication Infrastructure: Networks, cyber-physical systems and protocols that enable data transmission between the physical asset and its digital twin.
    \item Data Processing and Storage: Systems for processing and storing large amounts of data.
    \item Analytics and Intelligence: Advanced analytics, AI, and machine learning algorithms for data interpretation and decision-making.
    \item Visualization and User Interface: Tools for visualizing the digital twin and interacting with it.
    \item Integration Frameworks: Software that integrates the digital twin with other systems and applications.    
\end{enumerate}

A cyber-physical system (CPS) can be considered a component of a digital twin. In the digital twin framework, CPS plays a crucial role as it represents the integration of computing, networking, and physical processes. The digital twin uses data from the CPS to create a virtual representation that can simulate, analyze, and predict the behaviors of its physical counterpart. This symbiotic relationship allows for real-time monitoring and advanced analytics, enhancing the capabilities of digital twins in various applications.


Generative AI, including Generative Adversarial Networks (GANs), can significantly benefit explainable AI (XAI) applications in various ways:

    Data Augmentation and Simulation: GANs can generate realistic, synthetic data that can be used to train other AI models. This is especially useful in fields where real data is scarce or sensitive. By using GANs to generate data, researchers and developers can create more robust and diverse datasets, leading to better model training and explanation of how the model behaves with different types of data.

    Feature Visualization and Understanding: GANs can be used to visualize and understand complex features learned by deep neural networks. For example, GANs can generate images that maximize the activation of certain neurons in a network, helping to understand what features the network is paying attention to.

    Counterfactual Explanations: GANs can create counterfactual examples, which are essentially "what-if" scenarios. These counterfactuals can help in explaining decisions made by AI systems. For instance, by altering input data slightly and observing how the AI's output changes, one can gain insights into the decision-making process of the AI.

    Model Robustness and Testing: GANs can be used to test the robustness of AI models by generating adversarial examples. These are inputs that are specifically designed to fool the AI model. Understanding how and why a model is fooled by these adversarial examples can provide insights into the model's weaknesses and strengths, leading to better explanations of its behavior.

    Interpretable Feature Learning: GANs can be designed to learn more interpretable features. By constraining a GAN to learn representations that are more aligned with human-understandable concepts, the explanations derived from these models can be made more accessible to users.

    Benchmarking Explainability: GAN-generated data can serve as a benchmark for testing and comparing different explainable AI methods. Since the data and its characteristics are well-understood, it provides a controlled environment to assess the effectiveness of various XAI techniques.

    Human-AI Collaboration: By generating visualizations or simulations that are understandable to humans, GANs can facilitate better collaboration between humans and AI systems. This is especially important in fields like medicine or autonomous driving, where human experts need to trust and understand AI decisions.

    Enhancing Transparency: Finally, by providing tools to visualize, simulate, and test AI models, GANs contribute to the overall transparency of AI systems. This is a key component of explainable AI, as transparency is crucial for building trust and understanding in AI applications.

In summary, GANs and generative AI can play a crucial role in enhancing the explainability of AI systems by providing tools for data augmentation, feature understanding, creating counterfactuals, testing model robustness, learning interpretable features, benchmarking XAI methods, aiding human-AI collaboration, and enhancing overall transparency.


, five challenges that remain to be addressed are further provided along with promising future perspectives. This survey will help the reader better understand how the GAN is employed in the transportation domain and offer useful suggestions for the future development of the framework.

Aiming at improving the efficiency of traffic anomaly inspection, we exert effort towards defect detection on roads and bridges, railway defect inspection, and traffic anomaly monitoring. 



Traffic flow research emphasizes spatio-temporal data forecasting and sparse data completion, both of which can be improved by GAN-based models. Commonly-used model evaluation indices are additionally mentioned in this part.

==> Content/02-title-authors.tex <==
\title{ \rev{Leveraging Generative AI for Urban Digital Twins: A Scoping Review on the Autonomous Generation of Urban Data, Scenarios, Designs, and 3D City Models for Smart City Advancement}}

%\title{Leveraging Generative AI for \rev{Smart Cities and Urban} Digital Twins: A Survey on the Autonomous Generation of Data, Scenarios, 3D City Models, and Urban Designs}

%\tnotetext[t1]{This manuscript has been co-authored by UT-Battelle, LLC, under contract DE-AC05-00OR22725 with the US Department of Energy (DOE). The US government retains and the publisher, by accepting the article for publication, acknowledges that the US government retains a nonexclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this manuscript, or allow others to do so, for US government purposes. DOE will provide public access to these results of federally sponsored research in accordance with the DOE Public Access Plan (http://energy.gov/downloads/doe-public-access-plan).}

\author{Haowen Xu} 
\ead{xuh4@ornl.gov}
\author{Femi Omitaomu\corref{cor1}}\ead{omitaomuoa@ornl.gov}
\author{Soheil Sabri} \ead{soheil.sabri@ucf.edu}
\author{Sisi Zlatanova} \ead{s.zlatanova@unsw.edu.au}
\author{Xiao Li} \ead{xiao.li@ouce.ox.ac.uk}
\author{Yongze Song} \ead{Yongze.Song@curtin.edu.au}


\cortext[cor1]{Corresponding author.}

\address[CSED]{Computational Urban Sciences Group, Oak Ridge National Laboratory, Oak Ridge, TN 37830, USA}
\address[UCF]{Urban Digital Twin Lab, School of Modeling, Simulation, and Training, University of Central Florida , 3100 Technology Parkway,  Orlando, 32826 FL, USA}
\address[UNSW]{GRID, School of Built Environment, UNSW Sydney, NSW 2052 Australia}
\address[Oxford]{Transport Studies Unit, University of Oxford, South Parks Road, Oxford, OX1 3QY, UK}
\address[Curtin]{School of Design and the Built Environment, Curtin University, Kent St, Bentley WA, AU}


 
% \author{
% \IEEEauthorblockN{Pablo Moriano\IEEEauthorrefmark{1}\printfnsymbol{2}\thanks{\printfnsymbol{2}Corresponding author.},~\IEEEmembership{Senior Member,~IEEE}, Andy Berres\IEEEauthorrefmark{3},~\IEEEmembership{Member,~IEEE}, Haowen Xu\IEEEauthorrefmark{3},~\IEEEmembership{Member,~IEEE}, Jibonananda Sanyal\IEEEauthorrefmark{4},~\IEEEmembership{Member,~IEEE}
% } \\
% \IEEEauthorblockA{\IEEEauthorrefmark{1}Computer Science and Mathematics Division, Oak Ridge National Laboratory; \IEEEauthorrefmark{3}Computational Sciences and Engineering Division, Oak Ridge National Laboratory; \IEEEauthorrefmark{4}National Renewable Energy Laboratory\\
% $\{$moriano, berresas, xuh4$\}$@ornl.gov, jibo.sanyal@nrel.gov}
% }

\makeatletter
\newcommand{\printfnsymbol}[1]{%
  \textsuperscript{\@fnsymbol{#1}}%
}

% In-house commands
\newcommand*{\MyIndent}{\hspace*{0.5cm}}%

%\linenumbers


==> Content/Original/30-applications-origin.tex <==
\section{Generative AI in Smart City Applications} \label{sec:Dataset}
This section will provide a structured review of how the recent advancements in generative AI are revolutionizing key areas of urban science research and smart city applications, including traffic and transportation management, mobility research, building operations, energy management, and infrastructure planning. We primarily focus on the applications of the Generative AI models, including GANs, VAEs, transformer-based models, and generative diffusion models. The following subsections will delve into specific application areas of Generative AI models in each of the mentioned smart city areas (as depicted in Figure \ref{fig:overview}) to highlight their transformative ability to address challenges in urban digital twin applications.

\begin{figure*}[htb]
 \centering
\includegraphics[width=\textwidth]{Figures/generative_ai_overview.png}
 \caption{Generative AI application areas in major smart city sectors.}
 \label{fig:overview}
\end{figure*}

\subsection{Data Augmentation} 
\label{subsec:data-augmentation}
Data augmentation refers to techniques used to increase the amount of data by adding slightly modified copies of already existing data or newly created synthetic data from existing data \citep{lemley2017smart}. This is particularly common in machine learning and deep learning, where more training data leads to better model performance. Data augmentation is primarily about creating additional data points to improve the robustness and accuracy of models in tasks like image recognition, classification, and predictions \citep{moreno2020improving}. Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs) are prevalent in smart city applications for data augmentation, given their proficiency in generating high-quality synthetic data. However, generative diffusion models, known for their strengths in denoising and data augmentation, are primarily utilized in medical research rather than urban science. This suggests a potential untapped area for these models in urban applications, where their unique capabilities could offer novel solutions to complex urban challenges.
 
\subsubsection{Mobility and Transportation Management}
Generative AI plays a crucial role in transforming transportation and urban mobility management by leveraging data augmentation techniques. It enhances the accuracy and reliability of predictive models, enabling more efficient traffic flow, route optimization, and smart city planning by generating realistic, varied datasets that mimic complex urban environments.

\citet{zhou2021improving} introduces the Trajectory Generative Adversarial Network (TGAN) to address challenges in identifying and linking human mobility patterns, particularly in location-based social networks (LBSNs). By combining adversarial learning and spatio-temporal data analysis, TGAN significantly enhances trajectory-user linking (TUL) by generating synthetic trajectories that closely mimic real human movement patterns. This approach effectively overcomes issues of data sparsity and imbalanced label distribution in trajectory data, demonstrating superior accuracy in TUL compared to existing methods. The use of GANs for data augmentation in this context marks a substantial advancement in human mobility analysis, offering promising implications for various applications, including urban planning and personalized services. \citet{jilani2022traffic} presents an innovative approach to traffic congestion analysis using GANs for data augmentation. The research introduces a five-layer convolutional neural network model that leverages GAN-enhanced datasets for improved accuracy in classifying traffic congestion. This method significantly improves identifying congestion patterns, achieving a 98.63\% accuracy rate. The study highlights the efficacy of GANs in generating realistic synthetic images, thereby enriching the dataset for more effective traffic management and planning applications. \citet{dabboussi2023gan} explores an innovative approach using GANs for data augmentation in traffic management. The study presents a novel GAN-based model that successfully generates synthetic traffic data, addressing the critical issue of data scarcity in Intelligent Transportation Systems (ITS). This method demonstrates a significant improvement in traffic prediction models, enhancing their performance through the addition of realistic, GAN-generated data. The research contributes to developing more intelligent and sustainable transportation systems, underlining the potential of GANs in transforming ITS applications. \citet{islam2021sensor} presents a novel data augmentation technique using a VAE for improving transportation mode classification with limited training data. The VAE's decoder is adept at generating synthetic data that closely resembles real smartphone sensor data, effectively enlarging the dataset for machine learning models. This method enhances classification accuracy and addresses the imbalance in datasets by boosting underrepresented classes. Its application in activity recognition using smartphone sensors holds significant potential for vehicle-to-pedestrian (V2P) systems and smart mobility solutions. \citet{islam2021applying} presents novel deep learning applications in urban transportation systems. It showcases the use of VAEs and GANs for augmenting data in scenarios with limited datasets. The study highlights the capability of these deep learning models to generate synthetic data, which closely resembles real-world data, thus enhancing model training and predictive performance in transportation applications like crash data analysis and traffic pattern prediction. \citet{islam2021crash} introduces a VAE-based data augmentation technique to balance crash and non-crash event datasets in traffic systems. Due to the extreme imbalance in these datasets, traditional machine learning models tend to underperform. The VAE encodes events into a latent space, enabling the generation of synthetic crash data that statistically mirrors real data. This method outperforms traditional oversampling techniques like SMOTE and ADASYN, improving specificity and sensitivity in crash prediction models. It also addresses overfitting issues, showcasing VAE's capability in generating precise, balanced datasets for effective machine learning applications in traffic safety.

\subsubsection{Urban Energy Systems}
Data augmentation techniques, aided by generative AI, are increasingly pivotal in building energy modeling and power grid applications. These innovative methods have significantly enhanced the accuracy of predictions and forecasting, thereby streamlining the management of urban energy systems. 

\citet{wu2021gan} presents a novel approach to forecasting energy consumption using a GAN-enhanced ensemble model. This method combines GANs with ensemble learning, demonstrating significant improvements in forecasting accuracy. The study explores the use of GANs for data augmentation, which effectively enriches the training dataset with high-quality, diverse samples. This approach enhances the model's robustness and generalization capabilities, showcasing the utility of GANs in improving predictive models in energy management systems. The \citet{boicea2022novel} explores using GANs for augmenting data in power load forecasting. It demonstrates GAN's capability to expand a dataset, enhancing the predictive accuracy of a Convolutional Neural Network model used for load forecasting. This approach addresses the challenge of limited sample size in power load forecasting, showing GANs' effectiveness in data augmentation and their potential in improving forecasting accuracy in energy management systems. \citet{fan2022novel} utilizes deep learning, specifically deep generative modeling, for data augmentation in building energy prediction. This approach significantly improves the accuracy of short-term energy predictions in buildings. The study leverages the capabilities of deep learning to generate synthetic but realistic energy data, addressing the challenge of limited high-quality training data. This innovation demonstrates the potential of deep learning in enhancing data-driven models for smart building operation management, especially in scenarios with data scarcity.

\subsubsection{Building and Infrastructure Management}
Data augmentation, facilitated by generative AI, significantly enhances the predictive analytics and decision-making processes in building and infrastructure management \citep{baduge2022artificial}. Its application spans a broad spectrum, from structural detection to maintenance forecasting. 

\citet{abdollahi2020building} presents a groundbreaking approach in urban planning by integrating GANs, Genetic Optimization Algorithms (GOAs), and Geographic Information Systems (GIS). This study underscores the capability of deep learning, particularly GANs, in generating complex, high-dimensional urban building images. The innovative use of GANs for data augmentation, combined with the optimization strength of GOAs and the spatial analysis of GIS, demonstrates a novel framework in urban planning, enhancing efficiency, scalability, and decision-making in urban development.
\citet{li2023machine} addresses a significant challenge in the Structural Health Monitoring (SHM) of civil infrastructure using machine learning (ML), where a lack of comprehensive datasets for training models under various structural damage conditions is a common issue. To overcome this, the research introduces a novel data augmentation strategy within a vibration-based SHM framework, employing a Conditional Variational Autoencoder (CVAE). The CVAE is used to generate additional data samples of power cepstral coefficients of structural acceleration responses in diverse damage scenarios. This is achieved by training the CVAE to model different statistical distributions of these coefficients, using newly defined conditional variables. Notably, the decoder of the CVAE, once trained, is then used independently for the generation of new samples, enhancing the data augmentation process.
\citet{hoeiness2021positional} utilizes augmented GANs for predicting wind flow in urban environments. This innovative approach rephrases the problem of 3D flow fields into a 2D image-to-image translation challenge. The study explores the use of GANs, particularly Pix2Pix and CycleGAN, along with U-Net autoencoders, demonstrating GAN's ability to model complex spatial relationships and generate accurate wind flow predictions. This research represents a significant advancement in urban planning and pedestrian comfort analysis for improving street and infrastructure design.

By generating comprehensive datasets that replicate a vast array of environmental and usage conditions, these AI models empower the development of robust solutions, including innovative designs and optimization strategies. Their applications lead to more resilient and efficient operations and maintenance of buildings and urban infrastructure.

\subsection{Data synthesis and Scenario Generation} 
\label{subsec:scenario-generation}
Synthetic data generation involves artificially creating entirely new data that mimics real-world data and is different from data augmentation, which modifies existing data to create variations for enhancing the size and diversity of data sets for training data models \citep{figueira2022survey}. Popular generative AI models like GANs and VAEs are instrumental in synthetic data generation for smart city and urban research, offering diverse, realistic datasets where real data is scarce or sensitive due to privacy issues.
In many smart city applications, synthetic data supports scenario generation and analysis, enabling planners to simulate and predict outcomes of future and hypothetical urban developments, traffic patterns, and public services in a controlled and risk-free environment, thereby informing more effective and sustainable urban strategies. This approach leads to a more informed and effective scenario-based planning approach, facilitating the evaluation of potential impacts and outcomes of urban policies or changes before they are implemented in the real world.
 
\subsubsection{Mobility and Transportation Management}
In human mobility studies, generative models are widely used to generate synthetic trajectories that can realistically reproduce mobility patterns, as well as to enable predictions of future mobility patterns. \cite{luca2021survey} have provided a comprehensive survey on the generative AI applications for creating synthetic trajectories. As examples, \citet{smolyak2020coupled} innovatively uses GANs for anomaly detection in human mobility data. The authors introduce the Infinite Gaussian Mixture Model (IGMM) coupled with bidirectional GANs (BiGANs), an approach that generates realistic synthetic human mobility data and effectively detects multimodal anomalies. This method marks a significant advancement in anomaly detection, addressing the challenges of multimodal data patterns in human mobility and improving the accuracy of identifying anomalous behaviors or trajectories.
\citep{kosaraju2019social} presents a novel approach to pedestrian trajectory forecasting. It integrates a graph-based GAN with a graph attention network (GAT) and Bicycle-GAN to generate realistic multimodal trajectory predictions as future scenarios. This method effectively models the social interactions of pedestrians and accounts for the multimodal nature of human movement. The research demonstrates significant advancements in trajectory forecasting, contributing to applications like autonomous vehicle navigation and urban planning. 
\citep{huang2019variational} utilizes a Sequential Variational Autoencoder (SVAE) for reconstructing human mobility trajectories. This approach is novel in its integration of a Variational Autoencoder (VAE) with a sequence-to-sequence model, enabling the efficient capture of salient features in human mobility data. The SVAE model demonstrates the capability of VAEs in approximating complex, high-dimensional distributions like urban mobility patterns. This innovation is crucial for enhancing trajectory reconstruction in urban planning and intelligent transportation systems, addressing challenges of data sparsity and privacy concerns. \citet{bao2020covid} introduces an innovative approach using Conditional GANs to estimate human mobility during the COVID-19 pandemic. This research significantly contributes by addressing the challenge of estimating human mobility in rapidly changing social contexts with limited training data. The study employs a domain-constraint correction layer within the GAN's generator, enhancing the learning process and improving the quality of generated mobility predictions. This method demonstrates the potential of GANs in generating reliable spatiotemporal mobility data under uncertain and dynamically changing conditions, a crucial advancement in predictive modeling during public health crises. \citet{wang2020seqst} introduces SeqST-GAN, a model utilizing Sequence-to-Sequence (Seq2Seq) Generative Adversarial Networks for predicting urban crowd flow. It uniquely addresses the complex spatial-temporal correlations in urban environments by treating crowd flow data as sequences, akin to frames in a video. The combination of Seq2Seq and GANs enables the model to generate accurate multi-step predictions, overcoming the challenge of blurry predictions often seen in deep learning models. This innovative use of GANs demonstrates their capability in generating sequential, high-dimensional data, marking a significant advancement in urban planning and traffic management.

In many previous efforts that aim to develop intelligent transportation systems for efficient traffic planning and management, generative models are developed to create synthetic data for generating planning and simulation scenarios. As examples, \citep{wu2020spatiotemporal} explores the use of a Long Short-Term Memory (LSTM) network combined with GAN to generate traffic flow scenarios. This approach leverages the LSTM's capability in capturing temporal dependencies and GAN's strength in generating realistic traffic patterns. The innovation lies in accurately modeling and simulating complex traffic dynamics, aiding in traffic management and urban planning. This research highlights the potential of deep learning in enhancing predictive models for urban traffic systems. \citet{demetriou2023deep} utilizes GANs to create realistic driving scenarios for autonomous vehicle testing. This research demonstrates the innovative use of GANs in generating complex and diverse driving conditions, aiding in the development and validation of autonomous driving systems. The study highlights GAN's capability to simulate various road environments and traffic situations, which is crucial for ensuring the safety and reliability of autonomous vehicles in real-world conditions. \citet{mladenov2022adversarial} explores a novel application of GANs in traffic simulation. The study introduces an adversarial variational inference technique for calibrating Origin-Destination (OD) matrices in urban traffic simulators. This method is significant for its ability to mitigate the underdetermination problem in traffic simulation, leveraging GANs to match higher-order moments of field data. This innovative approach enhances the accuracy and robustness of traffic simulations, which is essential for effective urban traffic management and planning.


\subsubsection{Urban Analytics}
Generative AI models excel in creating realistic, high-dimensional data and data-driven scenarios that can mimic complex urban dynamics and processes based on realistic and historic data. By creating synthetic data and scenarios of various urban growth patterns, demographic distributions, and city layouts, these AI tools provide invaluable insights for urban planning, policy making, and morphology analysis, enabling researchers to explore diverse scenarios and predict future urban transformations effectively \citep{de2023geoai}. 

In terms of detail applications, \citet{johnsen2022population} explores the use of GANs for synthesizing realistic population datasets. This approach leverages GAN's capability to generate high-dimensional, diverse data, addressing the challenge of limited real-world demographic data availability. By creating synthetic populations that closely resemble actual demographics, the study showcases GANs' potential in urban planning and policy making, where accurate population models are crucial. \citet{kempinska2019modelling} explores the use of deep learning, specifically VAEs, in modeling urban street networks. It demonstrates how VAEs can effectively capture key urban network metrics in low-dimensional vectors and generate complex urban forms. This approach, capitalizing on the deep learning capability of generating realistic images, marks significant progress in data-driven urban modeling, leveraging the increasing availability of street network data to enhance the quantitative analysis of urban patterns. \citet{zhang2022metrogan} introduces Metropolitan GAN (MetroGAN), a novel Generative Adversarial Network framework, for simulating urban morphology with geographical knowledge. MetroGAN addresses limitations of previous GAN models such as data sparsity and training instability by incorporating a progressive growing structure and a geographical loss for water area constraints. It significantly outperforms existing urban simulation methods, demonstrating over 20\% improvement in all metrics. Interestingly, MetroGAN can generate city shapes using solely physical geography features, showcasing its ability to handle various urban attributes and stabilize GAN-based urban simulation. \citet{allen2022generative} delves into the application of deep learning, particularly GANs, for analyzing urban morphology. This research highlights the capability of GANs to process and interpret complex urban data, providing insightful analyses of city structures and patterns. The innovative use of GANs in this context offers significant contributions to urban planning and development, enhancing our understanding of urban spaces and their evolution. \citet{sun2021gan} explores land-use and land-cover change (LUCC) prediction using deep learning. It introduces a model employing GANs, specifically the pix2pix GAN, combined with an attention mechanism. This approach significantly enhances local spatial detail and diversity in urban planning and LUCC prediction. The model's unique capability lies in fusing multiscale local spatial information with city planning data to predict future land-use changes, showcasing a novel application of GANs in urban planning and environmental monitoring. \citet{kastner2023gan} presents an innovative GAN model for predicting urban wind flow. This GAN, designed for image-to-image translation, efficiently maps input urban geometry to predicted wind flow patterns. By utilizing Pix2Pix GAN, integrated with a voxelization process and distance-to-object encoding, the model offers rapid and accurate predictions of urban wind flow. This approach significantly reduces the computational cost and time associated with traditional Computational Fluid Dynamics (CFD) simulations, making it a promising tool for urban design and microclimate analysis.


\subsubsection{Urban Energy System}
Synthetic data supports the planning, management, and operation of urban energy systems by providing realistic, diverse datasets for modeling and simulating various energy scenarios\citep{li2020building, roth2020syncity}. These datasets can facilitate the optimization of energy distribution, demand prediction, and efficient resource allocation, reducing carbon-emission in cities and improving efficiency in grid systems.

As detailed examples, \citet{wang2020generating} introduces an innovative approach to generate realistic building electrical load profiles. Utilizing GAN, the research addresses the challenge of generating load profiles that accurately reflect dynamic and stochastic behaviors of real buildings. The study showcases GAN's capability to anonymize smart meter data, maintaining important statistical information while ensuring privacy. This advancement offers significant implications for smart meter data analytics, enhancing the integration of buildings with the electric grid and promoting sustainable energy management.
\citet{dong2022data} discusses a novel data-driven method for generating renewable energy production scenarios using controllable Generative Adversarial Networks (GAN). It focuses on addressing the challenges in power system planning and operation due to uncertainties in wind and solar energy. The proposed GAN model learns the stochastic and dynamic characteristics of renewable resources, enabling the creation of controllable, interpretable scenarios. This method enhances renewable energy modeling, offering significant contributions to the efficiency and reliability of power systems with high renewable penetration.
\citet{pan2019data} introduces an innovative application of deep learning in the field of electric vehicle (EV) load profiles generation. It employs a Variational Auto-Encoder (VAE), a deep learning model, to create EV charging load profiles. This approach is significant because it moves away from traditional methods that heavily rely on probabilistic models and manual data sampling. The VAE model, by learning the inherent characteristics of EV load data, generates diverse load profiles that accurately reflect temporal correlations and probability distribution of actual loads. This methodology signifies a noteworthy leap in using deep learning for more efficient and accurate energy management in the context of increasing EV usage.
\citet{jiang2018scenario} presents a novel approach for wind power scenario generation using GANs. This research stands out for its improvement of GANs, particularly in enforcing Lipschitz continuity through gradient penalty and consistency terms. These enhancements address common issues like overfitting and training instability, leading to more efficient and stable model training. The study demonstrates the effectiveness of this approach in generating high-quality scenarios for wind power, offering significant potential for renewable energy modeling and decision-making under uncertainty.
\citet{chen2018model} introduces an innovative approach for renewable energy scenario generation using GANs. This study highlights the ability of GANs to create realistic, data-driven scenarios, capturing the spatial and temporal correlations of renewable power plants. The method is particularly notable for its efficiency and scalability, offering a significant advancement in renewable energy modeling, especially for wind and solar power generation. This work demonstrates the potential of GANs in effectively handling the complexities and variabilities in renewable energy data.


\subsubsection{Urban Disaster Management}
Generative models, adept at synthesizing realistic images and scenarios, are being utilized for detecting particular disaster and simulating potential disaster impacts, enhancing preparedness strategies. In earthquake and flood management, for instance, GANs generate detailed images of damaged infrastructure, aiding in rapid damage assessment and efficient resource allocation \citep{tilon2020post}. This technology significantly improves response times and decision-making accuracy, proving vital in mitigating the effects of urban disasters and bolstering resilience in city planning and emergency responses. 

As detailed examples, \citet{hofmann2021floodgan} presents a novel deep learning approach for real-time pluvial flood prediction. The study introduces floodGAN, a deep convolutional generative adversarial network, which significantly accelerates flood prediction while maintaining high accuracy. This approach effectively utilizes the capabilities of deep learning, particularly GANs, to understand and predict complex flood dynamics based on spatially distributed rainfall events. The innovation lies in its ability to provide fast, accurate flood predictions essential for real-time applications such as early warning systems, marking a substantial advancement in flood modeling and risk management. \citet{salih2022comparison} explores the use of GANs and Mask Region-Based Convolutional Neural Networks (Mask-R-CNN) for floodwater detection and segmentation in images. The study highlights the capability of GANs to generate segmented images of flooded areas, emphasizing their potential in applications where quick and accurate floodwater identification is crucial. The research demonstrates the effectiveness of GANs in image-based flood detection, offering a novel approach to enhancing flood response and management strategies. \citet{yadav2024unsupervised} introduces an innovative unsupervised approach for flood mapping using Synthetic Aperture Radar (SAR) time series data. It leverages a Variational Autoencoder (VAE) trained with reconstruction and contrastive learning techniques. This model is adept at detecting changes by examining the latent feature distributions between pre-flood and post-flood data. Its performance, evaluated against nine different flood events, demonstrates superior accuracy over existing unsupervised models. This approach marks a significant advancement in the application of deep learning to environmental monitoring, specifically in enhancing flood detection capabilities using satellite data. \citet{lago2023generalizing} introduces cGAN-Flood, a conditional generative adversarial network developed to enhance flood prediction in urban catchments. Unlike traditional ANN models, cGAN-Flood can generalize flood predictions to areas outside its training dataset, addressing varying boundary conditions. It achieves this by using two cGAN models for identifying wet cells and estimating water depths, trained with HEC-RAS outputs. The method was tested on different urban catchments and compared with HEC-RAS and the rapid flood model WCA2D. It successfully predicted water depths, despite some underestimation in channels during low-intensity events. Significantly faster than existing models, cGAN-Flood offers a promising, efficient alternative for large-scale flood forecasting.
\citet{delacruz2020using} presents an innovative approach using GANs for rapid classification of earthquake-induced damage to railways and roads. It highlights the use of GANs to generate synthetic images of damage, addressing the challenge of limited real-world data for training deep learning models. This method demonstrates the potential of GANs in enhancing the efficiency and accuracy of structural damage assessment, which is crucial for emergency response and infrastructure recovery efforts. \citet{zhou2023automatic} utilizes GANs for urban morphology prediction related to local climate zones (LCZs). It employs GANs to integrate LCZ and urban morphology data from six cities, demonstrating superior accuracy and convergence capabilities, particularly with the Pix2pix model. This approach allows for rapid and responsive 3D urban morphology prediction, offering significant insights for enhancing local climates in urban areas through 3D generative design techniques.


\subsubsection{Urban Water Management} 
Currently, the applications of generative AI in urban water management is relatively limited, especially when compared to its broader use in other urban sectors. The primary focus of existing applications lies in the prediction and structural management of sewer water systems. This section will selectively explore and discuss a handful of pertinent examples in this domain. \citet{koochaligenerative} explores the innovative usages of GANs in urban water management, specifically in improving combined sewer overflow predictions, such as depth and flow rate. GANs are used for data augmentation, generating synthetic time series to balance datasets, thus enhancing the accuracy of prediction models. The study demonstrates that models trained with synthetic data generated by GANs can perform comparably to those trained with real data. The study proposed novel deep-learning approaches that can address challenges like data scarcity in urban water management. \citet{fu2022role} focuses on the application of GANs for tasks like predicting water system behaviors, improving operational efficiency, and enhancing decision-making processes. The paper underlines the effectiveness of GANs in handling complex, data-rich scenarios typical in urban water systems, demonstrating how these advanced AI models can contribute to more sustainable and effective water management strategies. \citet{situ2021automated} presents a novel approach for sewer defects detection. It utilizes state-of-the-art Style-based Generative Adversarial Networks (StyleGANs) to generate high-quality synthetic images of sewer defects. These images are then used to train and fine-tune seven well-known CNN models for automated sewer defects detection. The study demonstrates that both variants of StyleGANs are efficient in producing diverse and detailed images, significantly enhancing the performance of deep learning models in sewer defects detection.

%\subsection{Urban Data Enrichment} 
%This process involves enhancing, refining, or improving raw data. The key objective is to make data more valuable and insightful for analytical purposes. This is achieved by appending related information from external sources, correcting errors in the data, and updating outdated information. The enrichment process provides a richer context for analysis, helping in more accurate decision-making and insights.

\subsection{3D City Modeling} 
\label{subsec:3d-city}
The rapid advancement of City Digital Twins is propelled by digital infrastructure and ICT technologies linked to the Internet of Things (IoT), leading to the transformation of traditional cities into smart cities with enhanced infrastructure maintenance, socio-economic growth, and urban governance \citep{wang2021digital,caprari2022digital}. Among the majority of the existing digital urban twins, 3D city models has played a pivotal role to support the 3D modelling, monitoring and visualization of the smart city \citep{masoumi2023city}. 3D city models are also developed to enable the interactive and immersive visualization of complex urban environments to facilitate public engagement and collaborative urban planning \citep{dembski2019digital,xu2023toward}, simulation and evaulation of smart technologies \citep{xu2023semi,xu2023generative}, and 3D cadastral and urban design \citep{shojaei2013visualization, polys2018value}. 

Despite that the traditional geomatics and procedure-based methods \citep{lerma2010terrestrial,bejleri2021using} are capable of creating the Digital Surface Models (DSMs) of many large cities \citep{singh2013virtual}, these DSMs have limited resolution (e.g., texture and geometry) for representing building and infrastructure at the acceptable Level of Details (LoD). Additionally, many novel uses of 3D digital models (e.g., Hardware-In-the-Loop (HIL) simulations and scientific gamification) would require a gamified environment in which urban entities, such as buildings, roads, and infrastructure, are fully separated and have individual physical and gaming properties \citep{xu2023semi, xu2023toward}. In this setting, creating a high-fidelity 3D representation of a city is a challenging effort that often requires massive, repetitive, time-consuming and manual efforts for surveying and 3D modeling of urban entities \citep{xu2023toward}, along with advanced computing resources for processing and integrating large-scale GIS, remote-sensing (e.g., photogrammetry and LIDAR scan), and crowd-sourcing data in a virtual environment \citep{xu2023semi}. It has been an emerging trend to leverage the 3D content-generation capability of the recent generative AI techniques to automate the tremendous manual efforts for creating 3D assets of urban entities, such as terrain, buildings, infrastructures, and vegetation \citep{xu2023semi}. 

\subsection{3D Building Generation}
The autonomous capability of recent generative AI models has allowed them to create photo-realistic 3D representations of buildings and street environments\citep{pang20223d,wu2022generative}. These applications have advanced the technical capability of many urban science fields, including architecture design, building construction and operations, and urban planning.
\citet{Du_3d_building_gan} introduces a novel method for 3D building fabrication using a Hybrid GAN. This method incorporates a unique loss function, including cycle consistency and perceptual loss, and utilizes a multi-properties GAN chain to create complex architectural designs. It also features a mixed GAN network for generating geometry and texture coordination. This approach significantly enhances the realism of 3D building models, achieving a 20\% performance improvement over traditional methods, demonstrating its potential in applications like digital city construction and smart urban planning. 
\citep{kelly2018frankengan} discusses an innovative framework called FrankenGAN. This system is designed to enhance coarse building mass models by adding detailed geometric and texture details, creating realistic and visually appealing urban landscapes. FrankenGAN employs a cascade of Generative Adversarial Networks (GANs), synchronized to maintain consistent styles across multiple scales in neighborhoods. It offers user control over the variability of output styles through exemplar images, allowing for a blend of automated and user-guided design. This technology is significant for its potential to revolutionize urban modeling and architectural design, providing a powerful tool for researchers and professionals in these fields to generate detailed, large-scale 3D city models efficiently and with high fidelity. \citet{bacharidis20203d} explores the use of GANs for reconstructing 3D building facades from images. It employs deep learning techniques for facade structural element detection, depth point-cloud generation, and protrusion estimation. The study demonstrates GANs' capability in segmenting building components from images and generating detailed 3D facades. These capabilities show GANs' potential in evaluating urban scenes and extracting urban design parameters, such as window ratio, skyline, and other applications, including cultural heritage preservation. The approach aims to address the challenges of architectural diversity and data scarcity in 3D modeling.

\subsection{3D Street Environment Construction}
A few other studies have developed generative AI strategy to digitize the entire street environment (with buildings and infrastructure) as 3D models, laying an foundation for the next-generation extended reality applications for supporting participatory and collaborator urban design and planning \citep{xu2023toward}. 
\citet{tancik2022block} presents a significant advancement in neural rendering for large-scale urban environments. It introduces Block-NeRF, a variant of Neural Radiance Fields (NeRF), specifically designed to handle city-scale scenes. This method effectively decomposes a large scene into individually trained NeRFs, allowing for scalable rendering and enabling updates to specific parts of the environment without retraining the entire network. This technique represents a major step forward in the field of photorealistic 3D reconstruction and neural rendering.
\citep{kim2020citycraft} introduces a novel method for generating three-dimensional virtual models of cities from a single street-view image. This approach differs from traditional reconstruction methods by utilizing machine learning, specifically generative adversarial networks (GANs) and convolutional neural networks (CNNs), to create terrain maps and identify city components and styles. The generated 3D virtual cities are visually plausible and resemble actual cities. This method represents a significant advancement in the field of urban modeling, offering a unique and efficient way to create detailed, large-scale city models, which is particularly useful for applications in gaming, film, and urban planning. The use of GANs and CNNs in this context is notable for its ability to support research and development in these areas by providing a more streamlined and user-friendly approach to city modeling.



\subsection{Generative Urban Design and Optimization} 
\label{subsec:urban-design}
Generative design is defined as using computer-aided generative methods to produce design options, practices, and solutions, improving certain stages of the typical design process \citep{stojanovski2020city, buhamdan2021generative}.
In recent years, generative AI models play a crucial role as the intelligent agent in computer-aided urban design. They are employed in many studies of urban design alternatives and strategies that are driven by urban big data and previous solutions \citep{al2021generative}. The trend of publications that apply generative AI in urban design and optimization has been summarized in Figure \ref{fig:scopus-generative-urban-design}. Recent progress in generative urban design is evident in the urban science and smart city sector, where these models are increasingly used for tasks such as urban layout and land use optimization, environmental impact assessments, and urban resource management. 
At a high level, a study by \citet{quan2019artificial} highlighted the effectiveness of AI in managing urban complexity and sustainability, as well as supporting generative and participatory urban design. Furthermore, the integration of AI in smart cities is demonstrated by the work of \citet{batty2018artificial}, who emphasized AI's role in analyzing large-scale urban data to inform better city planning and management. The trend towards AI-aided urban planning signifies a paradigm shift, promising smarter, more efficient, and sustainable urban environments.

\begin{figure*}[htb]
 \centering
\includegraphics[width=\textwidth]{Figures/scopus_urban_generative_design.png}
 \caption{Summary of generative urban design and optimization publications using Scopus database (accessed on Jan 10th 2024)}
 \label{fig:scopus-generative-urban-design}
\end{figure*}

As examples of detailed generative urban design applications, \citet{huang2022accelerated} explores the use of GANs, in urban design for environmental performance optimization. It demonstrates the use of GANs in rapidly generating urban design alternatives that meet specific environmental criteria, highlighting deep learning's ability to process complex spatial data and simulate various urban development scenarios. This approach represents a significant innovation in integrating environmental considerations into the urban design process using advanced AI techniques.
\citet{fedorova2021generative} examines the use of deep learning, particularly GANs, in creating urban layout designs. It focuses on GANs' ability to generate diverse and realistic urban layouts, which can significantly aid in urban planning and development. This research underscores the potential of deep learning in addressing complex spatial design challenges, providing innovative tools for urban designers and planners.
\citet{noyman2020deep} explores the application of generative AI models, such as GANs and VAEs, in urban design, focusing on generating urban block layouts. This innovative approach does not require predefined parameters for design solutions, as the neural network learns the visual features of existing city structures. The research demonstrates GANs' ability to adapt designs to various urban contexts and morphologies. Significantly, it highlights the potential of generative AI in urban planning, offering a novel method for designing urban blocks that structurally align with the existing urban fabric without the need for explicit parameter definitions. It should be mentioned that social, economic, and environmental considerations can be used as constraints to improve the urban blocks from the livability and sustainability perspectives.
\citet{quan2022urban} develops Urban-GAN, an AI-aided generative urban design computation system, which empowers public participation in urban design through Generative Adversarial Networks (GANs) and Deep Convolutional Neural Networks (DCNNs). This innovative system enables individuals with little design expertise to generate professional-level urban designs. It employs sub-symbolic representation and case-based reasoning, facilitating users to select urban form cases and generate similar design schemes. The system's application in hypothetical design experiments across cities like Manhattan, Portland, and Shanghai illustrates its effectiveness in generating diverse urban forms, highlighting its potential in democratizing urban design and planning.
\citet{kimparticipatory} focuses on developing an AI tool called PlacemakingAI, which uses Generative Adversarial Networks (GANs) for urban design. The tool facilitates public participation in urban planning, allowing users to visualize sustainable urban spaces in real-time. It leverages both supervised and unsupervised GANs to generate synthetic images from datasets of walkable streets. This research is significant for its innovative use of GANs in urban design, enabling a participatory approach and fostering engagement from citizens, designers, and stakeholders in the urban design process.

==> Content/Original/40-futureDIscussion.tex <==
\section{Future of Generative AI in Urban Digital Twins} 
\label{sec:Future Discussion}
This section explores the integration of generative AI models with \rev{the existing} urban digital twin applications (e.g., web-based platforms, cyber-physical systems, \rev{and visual dashboards}), aiming to augment their current capabilities for more efficient \rev{participatory} smart city management \rev{through human-AI collaboration}. Additionally, we delve into the potential technical and methodological challenges associated with the development of generative urban digital twins, underscoring the complexities and innovations required for this visionary approach. 

\subsection{\rev{Cognitive Digital Twins: Visions and Opportunities}} 
As an integration between AI and digital twins, \rev{the emerging} Cognitive Digital Twins \rev{(CDTs)} represent a significant advancement in the digital twin concept, \rev{enabling self-learning, memory, and reasoning capabilities beyond their traditional counterparts \citep{niloofar2023general}. } These \rev{AI} models assimilate cognitive functions, enabling CDTs to dynamically process and learn from data. They harness deep learning to analyze complex datasets, predict future scenarios, and make decisions autonomously, leading to improved efficiency and adaptability \citep{ali2021cognitive}. In urban science and smart city applications, \rev{the CDT concept illuminates more intelligent, efficient, and automated solutions to complex urban management problems by leveraging the advanced capabilities of various neural networks for classification, fault detection, object detection, and optimization.}

\rev{Recent revolutionary advancements in GenAI can be integrated into CDT to further enhance its capability for more efficient and participatory urban management in the aspects of (a) facilitating data enhancement and enrichment, (b) building autonomous systems, and (c) promoting human-AI partnership. We present our vision of how GenAI models could be integrated into CDT for smart cities through Figure \ref{fig:dt-opportunities}, in which we adopted the core layers of a CDT defined by previous studies \citep{shi2022cognitive,abburu2020cognitwin} and elaborated on who individual layers could be benefited from GenAI through the following subsections. The essential layers of a CDT are represented by dark blue boxes, while our proposed visions and opportunities are depicted in green boxes in the figure.
} 

\begin{figure*}[htb]
 \centering
\includegraphics[width=\textwidth]{Figures/visions_opportunities.png}
 \caption{Potential opportunities of generative AI techniques for enhancing cognitive urban digital twins at the conceptual level.}
 \label{fig:dt-opportunities}
\end{figure*}


\rev{\subsubsection{Data Enhancement and Enrichment} }
\rev{Data quality and utility is critical to data-driven applications, especially urban digital twins that leverage urban data to enable the situational awareness, predictive analytics, and informed decision supports of various urban subsystems. 
\begin{description}
 \item[Data enhancement] refers to the augmentation of existing data sets by adding more detailed information, often from external sources, to make the data more comprehensive. In this context, Generative AI models, such as GANs and VAEs, have been widely utilized in contemporary studies to generate realistic data \citep{wu2022generative}, thereby enhancing the reliability and accuracy of a CDT's situational awareness capabilities. Additionally, VAEs are particularly effective in facilitating fault and anomaly detection, which further supports data enhancement efforts \citep{guo2020unsupervised}. VAEs operate by encoding input data into a latent space and then decoding it back to the original space, a process that enables them to capture complex data distributions and identify deviations from normal patterns. This ability to detect anomalies and generate synthetic data contributes to creating more robust and comprehensive datasets, ultimately improving the quality and utility of the data.  
 \item[Data enrichment] involves the integration of additional data to provide more context, making the data more meaningful and useful for analysis. In this regard, Generative AI models, such as GANs (Generative Adversarial Networks) and VAEs (Variational Autoencoders), have been frequently utilized in urban studies to generate synthetic data and simulate scenarios \citep{figueira2022survey}. 
\end{description}
The data synthesis capabilities of these models enhance an urban digital twin's predictive analytics, allowing for accurate projections and forecasts of urban dynamics in futuristic or hypothetical management scenarios. For instance, the design and development of critical infrastructure, such as airports, and their complex interactions with urban transportation systems can be modeled and simulated through various scenarios. By integrating proposed future developments (e.g., new buildings and transport networks) with current and real-time data (e.g., traffic patterns, existing buildings, and land uses), these models enable the creation of "what-if" scenarios. These scenarios provide digital twin users with alternatives for more adaptive and informed decision-making, ultimately supporting more resilient and efficient urban planning and management. 
By leveraging GenAI, urban digital twins can achieve more comprehensive, context-rich data, ultimately leading to more reliable data-driven insights and inferences, as well as more accurate predictive analytics. This enhancement enables opportunities for creating better-informed urban decisions and strategies.}

%\rev{Through data augmentation, generative AI techniques can With improved data quantity, quality, and realistic synthetic data that are generated based on real-world data, the urban digital twins' predictive analytics capability can be improved to predict or forecast the dynamics and response of different urban systems to either futuristic or hypothetical scenarios through data and physics-driven models. The ability of generative AI models to generate realistic data and codes in different programming languages can be applied to automate the software development of urban digital twins' components, such as 3D city models and scenario-based simulations (e.g., traffic, mobility, and building energy). This generative ability can significantly increase the adaptability and scalability of digital twin platforms by extending their coverage to new geographic areas and urban domains. For instance, the process of building development approvals, which involves structural, energy, and site examinations, can be automated.}

%\item[Enhancing Situational Awareness:] Through data augmentation, generative AI techniques can generate realistic urban data to refine the spatiotemporal resolutions and facilitate anomaly detection in the raw data, such as point clouds and satellite images \citep{wu2022generative}. Therefore, these techniques enhance the urban digital twins' capability to replicate the dynamics and reflect the state of the real-world urban systems in the digital environment.
%\item[Improving Prediction Accuracy:] With improved data quantity, quality, and realistic synthetic data that are generated based on real-world data, the urban digital twins' predictive analytics capability can be improved to predict or forecast the dynamics and response of different urban systems to either futuristic or hypothetical scenarios through data and physics-driven models. For instance, the design and development of critical infrastructure such as airports and their complex interactions with urban transportation systems can be modeled and simulated through different scenarios by integrating proposed future developments (e.g., buildings and transport networks) with current and real-time data (e.g.traffic, current buildings, and land uses). These "what-if" scenarios also provide alternatives to digital twin users for more adaptive decision support.

\rev{\subsubsection{Autonomous Systems} }
\rev{Recent developments in GPT and RAG have highlighted the potential for creating autonomous systems or agents to automate both data analytics and software development \citep{suri2023software}. Building an urban digital twin requires significant interdisciplinary efforts in data management, analysis, and software engineering. In this regard, integrating Generative AI models, particularly GPTs, can help automate labor-intensive, time-consuming, and repetitive tasks, thereby reducing the cost of developing and maintaining an urban digital twin. GenAI-powered autonomous systems can be deployed in the virtual and service layers of a CDT to generate computer code in various programming languages, facilitating the creation of core data analytics and software components.
}
\rev{
\begin{description}  
 \item[Autonomous Data Analytics] leverage GPTs' reasoning and generative capabilities to develop automated data workflows and pipelines that can perform advanced data analysis (e.g., statistical, mathematical, and spatial analysis) by calling appropriate libraries based on user-defined prompts \citep{vemprala2023chatgpt}. These autonomous systems often employ prompt engineering, predefined prompt bases and templates, and fine-tuning techniques to instruct large language models on specialized data analysis tasks. An example of an autonomous spatial analysis tool powered by the ChatGPT API is presented by \cite{li2023autonomous}. With the recent advancements in RAG, GPTs are now empowered with the capability to query external information sources through vector databases, broadening the application and utility of these generative models.   
 \item[Autonomous Software Development]  focuses on utilizing GPTs' code generation capabilities to develop critical software components \citep{suri2023software}. Numerous studies have explored GPTs' ability to create web applications, knowledge graphs, and databases using prompt templates and fine-tuning techniques \citep{liukko2024chatgpt,jamdade2024pilot,vamsi2024human}. Since urban digital twins are essentially web-based or cloud-based applications, their core software components could potentially be generated using GPTs and other pre-trained language models. Consequently, we envision an autonomous system for code generation as a component of the service layer in CDTs, designed to automate the time-consuming software development and maintenance tasks. The approach can generate codes for both the server-side and client-side applications. 
\end{description}
}
\rev{
Integrating GenAI-powered autonomous systems (i.e., agents) into a CDT can significantly lower the technical barriers and programming skills required for developing an urban digital twin. In terms of new application opportunities, this paradigm can reduce the costs associated with software development and maintenance while increasing the efficiency of domain experts, such as urban planners and researchers in academia with moderate coding experience, allowing them to develop robust urban digital twin applications. These autonomous systems facilitate the creation of specialized research software, including digital twins, decision support systems, and content management systems. Consequently, researchers can focus more on their domain expertise and less on technical implementation and software engineering practices.
}


% \item[\rev{GPT}-powered Autonomous System:] The integration of \rev{the large language} models, \rev{such as ChatGPT}, into software tools \rev{and development kits} is becoming increasingly popular, supporting \rev{the automation of various research tasks in multiple scientific domains. Example of these tasks include software development, autonomous analytics, data management and ontology creation.}

%Recent studies have demonstrated the potential of leveraging these models to develop autonomous systems \citep{li2023autonomous,vemprala2023chatgpt}. Such advancements aid in research and decision-making processes, addressing complex scientific challenges by combining GPT APIs with domain-specific data and simulation models. By employing APIs provided by GPT, \rev{in combination with various tuning techniques (), }researchers can seamlessly integrate generative AI capabilities into urban digital twins' various components. This integration facilitates \rev{automated} data integration, augmentation, and enrichment, enhancing AI-assisted urban design, education, decision-making, and the interpretation of intricate urban data and simulation models. This approach not only streamlines the incorporation of advanced AI technologies into urban planning and management but also opens new avenues for innovative, data-driven solutions to urban challenges.


%to foster a more efficient human-AI partnership, benefiting various participants in urban management processes, including domain experts, policymakers, technology providers, and city residents
%Within the proposed integration, the urban digital twin application serves as the cyberinfrastructure (i.e., information technology infrastructure) to ensure the collection, management, and provisioning of urban data and simulation outputs, which conceptualize and characterizes various urban subsystems and their dynamics through data and virtual layers. Within these layers, GenAI models' data augmentation and synthesis capability could further enhance the data and simulation scenarios by improving their data quality and accuracy. 
% while the GenAI models are responsible for augmenting the advanced features in the cognition layer. These advanced features are
%The vision of incorporating GenAI techniques in CDTs is to achieve an autonomous and generative system that will be cognitive, context-aware, fully automated, and cost-effective. This paper believes that the capability of previous generative AI applications reviewed in the previous section can be seamlessly integrated into cognitive urban digital twins. Future directions or opportunities for the generative urban digital twins are discussed as follows (as depicted in ).



%\begin{description}  
   %\item[Facilitating Human-AI Collaboration:] By generating visualizations, text, and data-driven insights that are understandable to humans, generative AI models can facilitate better collaboration between humans and AI systems. These models can be designed to learn more interpretable features, which are more aligned with human-understandable concepts derived from the domain knowledge. The explanations derived from these models can be made more accessible and sensible to digital twin users.

   %\item[Enabling Autonomous System Development:] The ability of generative AI models to generate realistic data and codes in different programming languages can be applied to automate the software development of urban digital twins' components, such as 3D city models and scenario-based simulations (e.g., traffic, mobility, and building energy). This generative ability can significantly increase the adaptability and scalability of digital twin platforms by extending their coverage to new geographic areas and urban domains. For instance, the process of building development approvals, which involves structural, energy, and site examinations, can be automated.   

   %\item[Supporting Decision Optimization:] Generative AI models can generate counterfactuals based on multiple "what-if" scenarios. These generated urban design or planning strategies can be used as alternatives to help urban planners evaluate the feasibility and efficiency of numerous planning or design alternatives and select the optimized solutions. This addresses the current gap in comprehensive impact analysis of urban design scenarios. This is due to the limitation of computational models and algorithms. For instance, in a Transit Oriented Development (TOD) scenario, different urban design analytics, including building height, sky view factor, walkability, and accessibility to different modes of transport, need to be evaluated. 

   %\item[Promoting AI-aided Design:] Generative models can rapidly generate a wide range of urban design concepts based on specific criteria or policy (e.g., walkability, accessibility, safety, and security, climate resilience), helping planners explore creative ideas and inspirations that might not be immediately visible to humans. Additionally, these models can tailor and modify existing human designs to meet a community's or environment's specific needs, and suggest design elements that are more likely to be successful in a particular area.      
%\end{description}

\rev{\subsubsection{Human-AI Partnership} }
\rev{
In the CDT's cognition layer, where human involvements are often required to make critical decisions, GenAI models and their generative abilities can be harnessed to promote human-AI partnerships for a more participatory, adaptive, collaborative urban management approaches, which match the demanded and skills of various participants in urban managements. These participants include domain experts (e.g., urban planners and researcher), policymakers, and city residents. The proposed approaches are centered are around two aspects, namely conversational AI for decision support and GenAI-aided co-design.
}
 
\rev{
\begin{description}  
 \item[Conversational AI] refers to emerging AI agents powered by advanced large language models, such as GPT, which enable intuitive and interactive communication between human users and AI systems \citep{mctear2022conversational}. Unlike traditional expert systems that often require users to possess domain knowledge, conversational AI offers a more natural, intuitive, and user-friendly interface. This allows individuals to participate in decision-making processes informed by data-driven insights, domain-specific simulations, and AI-powered predictive analytics \cite{sakirin2023user}. Conversational AI paradigms have proven effective in facilitating public engagement and participation in urban planning and management \citep{sahab2024conversational}. By providing a GPT-powered medium with excellent language understanding capabilities, these systems eliminate the need for users to have domain expertise. This approach enables interactive, user-centered dialogues with city residents and policymakers, capturing their needs and providing education and information relevant to support informed decisions. By integrating conversational AI into urban digital twins, GenAI promotes a more interactive, efficient, and democratic decision-making process, ultimately leading to more resilient and adaptive urban environments.  
 \item[GenAI-aided Co-Design] can revolutionize urban planning and management by enabling more dynamic, collaborative, and innovative approaches to city development and management. GenAI models assist in co-design processes by interpreting and responding to user inputs, allowing stakeholders to collaboratively explore various planning scenarios and design alternatives. Leveraging the generative capabilities of models such as GANs, VAEs and generative diffusion models, trained on successful design blueprints and practices, domain experts (e.g., urban planners and researchers) can automate the creation of urban designs (e.g., floor plans, street layouts, landscapes, and parks) across large geographic regions in a short period of time \citep{guridi2024image, quan2022urban}. This paradigm not only lowers costs but also enables urban planners to formulate design problems and explore more options through AI-Generated Content (AIGC) \citep{jiang2023generative}. Furthermore, GenAI-powered tools facilitate co-design processes by allowing stakeholders, including community members, policymakers, and architects, to interact with AI systems through intuitive interfaces. This interaction can include generating and visualizing different design alternatives, optimizing layouts for sustainability and efficiency, and integrating inquiries and feedback in real-time \citep{knight2023generative}.
 \end{description}
}

\rev{By integrating GenAI models into urban digital twins, we can create opportunities for generating more inclusive, adaptable, and responsive solutions to the evolving needs and values of various urban management participants. These generative approaches not only enhances the quality and sustainability of urban environments but also empowers communities to play an active role in shaping their future by building transparent and trustworthy human-AI partnership. }


\subsection{GenAI-Digital Twin Integration: \rev{Technical Strategies} }

\begin{figure*}[htb]
 \centering
\includegraphics[width=\textwidth]{Figures/Figures_AI_DT_integrate.pdf}
 \caption{Technical strategies for AI-Digital Twin integration: Generative (Gen)-AI models deployment in different digital twin architecture. }
 \label{fig:dt-ai-integration}
\end{figure*}

\rev{This subsection explores potential technical implementation strategies for integrating popular GenAI models into existing urban digital twin applications.}
Through the evolution history of the urban digital twins, a few software architectures emerge as particularly adept at fostering sophisticated, scalable, and efficient digital representations of urban landscapes. Among these, monolithic architecture, microservices, and edge-computing architecture are pivotal \citep{ferko2022architecting}. Monolithic architecture lays the groundwork by facilitating interoperable services that communicate across a network and is crucial for developing basic cyberinfrastructure for amalgamating diverse simulation systems and data sources using the traditional server-client paradigm \citep{gos2020comparison}. Evolving from monolithic architecture, microservices architecture advances this model by organizing applications into collections of loosely coupled services that are often adopted in large-scale cloud-based applications. This structure promotes agile development and deployment of complex cyberinfrastructure systems, enabling seamless updates and scalability for specific elements (e.g., simulation models for specific urban subsystems) of an urban digital twin without impacting the overall framework \citep{ponce2019migrating,xu2023smart}. 
Meanwhile, Edge computing introduces a move towards decentralized and distributed data processing, allocating computational tasks nearer to the data origins at the network's edge nodes \citep{yu2017survey}. Examples of these edge nodes are often edge servers that are directly connected to sensors and mobile IoT devices for sensing various types of urban data \citep{xu2022mobile,marjanovic2018edge}. This shift is vital for urban digital twin development, as it allows for real-time data analysis and immediate response critical for the effective management of dynamic urban activities. Collectively, these architectural strategies create a formidable foundation for constructing urban digital twins, delivering the adaptability, scalability, and immediacy required to simulate and manage complex urban systems accurately.

To effectively integrate \rev{genAI-powered applications} within urban digital twins—often manifested through web-based platforms, cyberinfrastructures, and cloud computing services for enhanced smart city functionalities—we propose several technical strategies (as demonstrated in Figure \ref{fig:dt-ai-integration}). These strategies are designed to bolster scalability, performance, and precision in the AI-digital twin synergy. Tailored specifically to accommodate urban digital twins, these approaches are aligned with distinct architectural patterns. This ensures that each strategy not only addresses the unique challenges of integrating AI into these complex systems but also leverages the inherent strengths of the chosen architectural framework. By doing so, our approach facilitates the creation of dynamic, responsive urban digital twins that can evolve with the changing needs of smart city ecosystems.

\begin{description}
    \item[\rev{GenAI} as a Service:] To integrate AI models into digital twins that adopt monolithic architecture and microservices architecture, a reliable practice would be hosting these models as web services following the paradigm of the service-oriented architecture \citep{schnicke2020enabling}. Currently, many cloud computing platforms provide the foundational infrastructure needed for deploying ML and DL models as web services at scale, offering flexible resources and cyber-deliver capability that can dynamically adjust to the computational demands of \rev{GenAI}. Utilizing the recent containerization technologies, such as Docker, and orchestration tools like Kubernetes can further enhance scalability and manageability by allowing AI components to be deployed as microservices. This modular approach facilitates the seamless integration of \rev{GenAI} models into existing urban digital twin frameworks, ensuring that complex data-driven simulations and data analyses run efficiently across distributed computing environments.
    
    \item[Ad-hoc Data Processing and Analytics at Edge Nodes:] For urban digital twin applications that involve real-time data streaming and simulation capabilities, deploying \rev{GenAI} models on the edge nodes can reduce latency and bandwidth use by processing data closer to the data source (e.g., sensors and IoT devices), which is crucial for real-time applications like traffic flow optimization, building and grid operations, or emergency response simulations within urban digital twins. \rev{GenAI} models can be readily deployed on edge servers or data loggers that are directly connected to urban sensors for processing and distributing raw data. This practice is complemented by the use of data streaming and real-time analytics platforms, such as Apache Kafka and Apache Spark, which can handle the high-velocity data feeds sensed from urban environments and provide the necessary processing power to augment and enrich urban data for supporting enhanced situational awareness and simulation-based predictive analytics in real-time.

     \rev{\item[GPT Prompt Base and Templates for Smart Cities:] The emerging concept of GPT Prompt Template Base involves developing structured templates and foundational setups that guide Generative Pre-trained Transformers (GPT) in generating accurate and contextually relevant outputs. These templates include predefined patterns and placeholders that can be filled with specific information, ensuring consistency and efficiency in prompt creation. By facilitating the autonomous generation of data and code, GPT Prompt Template Bases can significantly streamline the development of urban digital twins. They enable domain experts, such as urban planners and researchers, to easily generate complex data analyses, predictive models, and software components for an urban digital twin without extensive programming expertise. This is particularly important for urban sciences and management, where the integration of diverse datasets and the need for rapid, adaptive decision-making are critical. Creating robust GPT Prompt Template Bases for these fields ensures that AI-generated content is reliable, relevant, and aligned with the specific needs of urban development and management, ultimately enhancing the effectiveness and scalability of urban digital twin applications.}     
\end{description}


\subsection{Challenges and Limitations} 
Although numerous \rev{GenAI} approaches have been developed to address challenges across different sectors of smart cities, significant obstacles persist. These challenges are often linked to the limitations of the generative AI models themselves or stem from technical issues related to integrating AI with urban digital twins.

\begin{description}
\item[Inherent Model Instability:] Generative AI models, such as GANs, often face difficulties in the data training processes to make these models reach a stable state where the generator and discriminator are well-balanced. This instability can manifest in several ways, including mode collapse, non-convergence, vanishing gradients, hyper-parameter sensitivity, and divergence \citep{sajeeda2022exploring,saxena2021generative}.

\item[Evaluation of AI-Generated Data:] The quality of AI-generated data is influenced by several complex factors, including the absence of objective evaluation criteria, challenges in detecting mode collapse, the lack of benchmark data, and issues arising from imbalanced data \citep{saxena2021generative}. Furthermore, there is a notable lack of consensus regarding assessment indicators for various types of AI-generated data, such as time series and spatial data. This ambiguity in evaluation standards can be attributed partly to the limited number of published studies in this area, which restricts the development of universally accepted benchmarks and metrics. %This gap in research highlights the need for more extensive and focused studies to establish reliable and standardized methods for evaluating the quality of AI-generated data.

\item[Computing, Data Storage, and Latency:]
In the context of smart cities and urban digital twin applications, generative AI introduces substantial computational challenges, necessitating high processing power to facilitate complex simulations of urban systems and real-time data analytics. Moreover, these applications demand rapid and efficient data storage solutions to handle the extensive data volumes generated and processed, encompassing everything from sensor data to detailed environmental models. The seamless integration of these technologies requires robust, scalable computing infrastructures and sophisticated data storage systems, designed to support the relentless and intensive data streams inherent to smart urban environments. 

\item[Network Latency:]
The network latency associated with the data exchange for sending the data to generative AI models must be minimized to support real-time smart city functionalities that perform time-sensitive analytics and cyber-physical controls, such as traffic management optimization and incident detection. Addressing these demands often entails equipping urban digital twins with ample communication bandwidth and computational resources to process these AI models in real time, ensuring efficient and effective smart city operations. In fact, generative AI models, such as the VAE, can also be used for data compression, potentially addressing the network latency issues. 


\end{description}

==> Content/Table/table-0_bk.tex <==
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{scriptsize}
\begin{table*}[hbt]
\footnotesize
\caption{\rev{An overview of urban digital twin examples in various urban application areas.}} \label{tab:udt} 
\begin{tabular*}{\textwidth}{|p{3.4cm}|p{12.15cm}| }
%\begin{tabular}{lllll}
 \hline
 \multicolumn{1}{c}
 {\cellcolor{black!10}\textbf{Application Area}}  & 
 \multicolumn{1}{c}{\cellcolor{black!10}\textbf{Examples}} \\
\hline         
     \begin{description}
        \item[] 
        \item[] 
        \item[] 
        \item[Transportation and Mobility] 
     \end{description}
     & 
     \begin{description}
         \item[Traffic Simulation]             \citep{kuvsic2023digital,saroj2021development, xiong2022design}  
         \item[Traffic Control Optimization] 
            \citep{xu2023smart, kamal2024digital, kumarasamy2024integration}
         \item[Traffic Data Prediction]            \citep{hu2021digital, nie2023digital,kumar2018novel}
         \item[Connected Automated Vehicles] \citep{fan2022ubiquitous,du2021digital,ali2023review, wagner2023spat}
         \item[Traffic Safety]  
            \citep{irfan2024towards,fu2024digital, lv2022digital, wang2022digital,lv2022traffic}     
         \item[Transportation Asset Management]
            \citep{gao2021digital,wu2022digital,adibfar2022creation}
        \item[Advanced Driver-Assistance Systems]
            \citep{wang2022mobility,wang2020digital, schwarz2022role}
        \item[Parking Management] \citep{chomiak2023use, zou2023digital, liu2023cognitive, shao2022computer}
        %\item[Decision Support]
        %    \citep{saifutdinov2020digital,consilvio2023towards}                  
     \end{description}          
      \\ 
 \hline %below is the second row
     \begin{description}
        \item[]         
        \item[Urban Energy ] 
     \end{description} 
     & 
     \begin{description}
         \item[Grid Operation] \citep{jafari2023review, eGridGPT2024,sifat2023towards,nordzi2022real}
         \item[Energy Management] \citep{srinivasan2020urban, xu2024novel,francisco2020smart}
         \item[Anomaly and Fault Detection]  \citep{danilczyk2021smart, jain2019digital, joseph2018prediction}
         \item[Renewable Energy] \citep{xu2023novel, belik2023implementation, agostinelli2021cyber} 
     \end{description}
            \\     
 \hline  
    \begin{description}
        \item[]         
        \item[Urban Water] 
     \end{description} 
     & 
     \begin{description}
        \item[Smart Water Grid] \citep{wu2023high, ramos2023smart, giudicianni2020overview}        
        \item[Water Supply and Distribution]        
        \citep{conejos2020building, karmous2019foundations,martinez2021digital}
        \item[Drainage and Stormwater System] \citep{bartos2021pipedream, sharifi2024application}
        \item[Wastewater Management] \citep{hallaji2021digital, wang2024digital,jiang2022intelligent}       
     \end{description}
     \\    
 \hline
    \begin{description}
        \item[]         
        \item[Building and Infrastructure] 
     \end{description}  & 
    \begin{description}
        \item[Building Operation] \citep{zhao2022developing, hodavand2023digital, el2022development}
        \item[Building Information Modeling] \citep{qiuchen2019developing, sepasgozar2020lean, sacks2020construction}    
        \item[City Information Modeling] \citep{shi2023ontology, shariatpour2024urban, petrova2021digital}
        \item[Infrastructure Management] \citep{al2021digital, broo2022design, shirowzhan2020digital, abdeen2023citizen, yu2022digital}
     \end{description}    
    \\    
 \hline
    \begin{description}
        \item[]         
        \item[Urban Planning and Design] 
     \end{description}     
    & 
    \begin{description}
        \item[]         
        \item[] \citep{yang2021urban, schrotter2020digital, white2021digital, kumalasari2023planning, beckett2022smart, xu2023toward}
     \end{description} 
    \\
 \hline
\end{tabular*}
\end{table*}
\end{scriptsize}
